A Weyl geometric approach to the gradient-flow equations in information geometry

The gradient-flow equations with respect to the potential functions in information geometry are reconsidered from the perspective of the Weyl integrable geometry. The pre-geodesic equations associated with the gradient-flow equations are regarded as the general pre-geodesic equations in the Weyl integrable geometry.

==> geomdef.tex <==
%%%
%%%   Abbreviations
%%%
\newcommand\mc{\multicolumn}
\newcommand\pb{\pagebreak}
\newcommand\lb{\linebreak}
\newcommand\ds{\displaystyle}
\newcommand\ts{\textstyle}
\newcommand\scs{\scriptstyle}
\newcommand\scscs{\scriptscriptstyle}
\newcommand\ph{\phantom}
\newcommand\tx{\text}
\newcommand\mr{\mathrm}
\newcommand\bm{\mathbf}
\newcommand\dsum{\ds\sum}
\newcommand\lsum{\sum\limits}
\newcommand\dint{\ds\int}
\newcommand\T{{\tx{\normalshape\tiny\sf T}}}
\newcommand\etal{\emph{et al}\xspace}
\newcommand{\bt}{\begin{tabular}}
\newcommand{\et}{\end{tabular}}
\newcommand{\twoup}[2][c]{\bt{@{}#1@{}}#2\et}
\let\tup=\textup
\newcommand\nf{\normalfont}
%%%
%%%   Miscellany
%%%
\newcommand\Sref[1]{Section~\ref{#1}}
\newcommand\Fref[1]{Figure~\ref{#1}}
\newcommand\Tref[1]{Table~\ref{#1}}
\newcommand\propref[1]{Proposition~\ref{#1}}
\newcommand\Eref[1]{Eq.~\eqref{#1}}
\newcommand\hook{\mbox{\Large$\clrcorner$}\:}
\newcommand\Christ[2]{{\textstyle\left\{\!\genfrac{}{}{0pt}{}{#1}{#2}\!\right\}}}
\newcommand\smasha{\relax \mathpalette\msm@sh}
\newcommand\msm@sh[2]{\setbox0\hbox{$\m@th#1{#2}$}\ht0=.8\ht0 \leavevmode\box\z@}
\newcommand\overa[2]{\binrel@@{\mathop{\kern\z@#2}\limits^{#1}}}
\newcommand\lvec[1]{\overa{\leftarrow\kern-.5ex}{\smasha{#1}}}
\newcommand\rvec[1]{\overa{\rightarrow\kern-.5ex}{\smasha{#1}}}
\newcommand\bra{\langle}
\newcommand\ket{\rangle}
\newcommand\semicolon{\nobreak\mskip2mu\mathpunct{}\nonscript\mkern-\thinmuskip{;}%
\mskip6muplus1mu\relax}
\newcommand{\rd}{\mathrm{d}} % Roman d for differential
\newcommand{\re}{\mathrm{e}} % Roman e for exponential
\newcommand{\ri}{\mathrm{i}} % Roman i for imaginary number
\newcommand{\rj}{\mathrm{j}}
\newcommand{\rk}{\mathrm{k}}
\newcommand\RR{\mathbb{R}}
\newcommand\CC{\mathbb{C}}
\newcommand\HH{\mathbb{H}}
\newcommand\ZZ{\mathbb{Z}}
\newcommand\openone{\leavevmode\hbox{\small$1$\kern-3.5\p@\normalsize$1$}\xspace}
\newcommand\lfrac[2]{\text{$#1/#2$}}
\newcommand\sfrac[2]{\text{${}^{#1}\kern-.2em/\kern-.1em_{#2}$}}
\newcommand\overover[2]{\overset{\smash[b]{\hbox{\raise14\ex@\hbox{$\hidewidth #1\hidewidth$}}}}{\smash[t]{#2}}}
\newcommand\underunder[2]{\underset{\smash[t]{\hbox{\lower11\ex@\hbox{$\hidewidth #1\hidewidth$}}}}{\smash[b]{#2}}}
\newcommand\link{\text{\raise.15ex\hbox{$-$}}\ignorespaces}
\newcommand\linkII{\text{\raise.15ex\hbox{$=$}}\ignorespaces}
\newcommand\linkIII{\text{\raise.15ex\hbox{$\equiv$}}\ignorespaces}
\newcommand\fullcirc{\raisebox{-1\p@}{\Large$\bullet$}\xspace}
\newcommand\fullsqr{\mbox{\vrule height5\p@ width5\p@}\xspace}
\newcommand\dotted{\mbox{${\mathinner{\cdotp\cdotp\cdotp\cdotp\cdotp\cdotp\,}}$}\xspace}
\newcommand\dashed{\mbox{-\;-\;-\;-}\xspace}
\newcommand\broken{\mbox{-- -- --}\xspace}
\newcommand\longbroken{\mbox{--- --- ---}\xspace}
\newcommand\chain{\mbox{--- $\cdot$ ---}\xspace}
\newcommand\dashddot{\mbox{--- $\cdot$ $\cdot$ ---}\xspace}
\newcommand\full{\mbox{---\!---\!---}\xspace}
\newcommand\nula{\mc{1}{c}{0}}
%%%%%%%%%%%%%%%%%
%   Operators   %
%%%%%%%%%%%%%%%%%
\DeclareMathOperator\arccosh{arccosh}
\DeclareMathOperator\arcsinh{arcsinh}
\DeclareMathOperator\arctanh{arctanh}
\DeclareMathOperator\arccoth{arccoth}
\DeclareMathOperator\sech{sech}
\DeclareMathOperator\csch{csch}
\DeclareMathOperator\cov{cov}
\DeclareMathOperator\diag{diag}
\DeclareMathOperator\Div{Div}
\DeclareMathOperator\diver{div}
\DeclareMathOperator\Exp{Exp}
\DeclareMathOperator\erf{erf}
\DeclareMathOperator\grad{grad}
\DeclareMathOperator\gyr{gyr}
\DeclareMathOperator\id{id}
\DeclareMathOperator\Id{Id}
\DeclareMathOperator\ind{ind}
\DeclareMathOperator\Lie{Lie}
\DeclareMathOperator\rank{rank}
\DeclareMathOperator\Ree{Re}
\DeclareMathOperator\Res{Res}
\DeclareMathOperator\rot{rot}
\DeclareMathOperator\sign{sign}
\DeclareMathOperator\Sgn{Sgn}
\DeclareMathOperator\sinc{sinc}
\DeclareMathOperator\Span{Span}
\DeclareMathOperator\Stab{Stab}
\DeclareMathOperator\Sym{Sym}
\DeclareMathOperator\tr{tr}
\DeclareMathOperator\Tr{Tr}
\DeclareMathOperator\trace{trace}
\DeclareMathOperator\Trace{Trace}
\DeclareMathOperator\var{var}
\renewcommand\Re{\operatorname{\mathrm{Re}}}
\renewcommand\Im{\operatorname{\mathrm{Im}}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%   Special Notations   %
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\Ad{\mathrm{Ad}}
\newcommand\ad{\mathrm{ad}}
\newcommand\AdS{\mathrm{AdS}}
\newcommand\Aff{\mathrm{Aff}}
\newcommand\col{\mathrm{col}}
\newcommand\const{\mathrm{const}}
\newcommand\im{\mathrm{im}}
\newcommand\GL{\mathrm{GL}}
\newcommand\Gr{\mathrm{Gr}}
\newcommand\Mat{\mathrm{Mat}}
\newcommand\PGL{\mathrm{PGL}}
\newcommand\SL{\mathrm{SL}}
\newcommand\PSL{\mathrm{PSL}}
\newcommand\SO{\mathrm{SO}}
\newcommand\Sp{\mathrm{Sp}}
\newcommand\Spin{\mathrm{Spin}}
\newcommand\SU{\mathrm{SU}}
\newcommand\U{\mathrm{U}}
\newcommand\nD{\mbox{$\not\!\!D$}}
%%%
%%%   Measures
%%%
\newcommand\gC{\ifmmode\,^\circ\tx{C}\else$\,^\circ$C\fi\xspace}
\newcommand\wt{\ifmmode\tx{wt}\,\%\else wt\,$\%$\fi\xspace}
\newcommand\at{\ifmmode\tx{at.}\,\%\else at.\,$\%$\fi\xspace}
\newcommand\mol{\ifmmode\tx{mol}\,\%\else mol\,$\%$\fi\xspace}
\newcommand\vol{\ifmmode\tx{vol.}\,\%\else vol.\,$\%$\fi\xspace}
\newcommand\mass{\ifmmode\tx{mass}\,\%\else mass\,$\%$\fi\xspace}
\newcommand\mm{\ifmmode\mu\tx{m}\else$\mu$m\fi\xspace}
\newcommand\ms{\ifmmode\mu\tx{s}\else$\mu$s\fi\xspace}
\newcommand\mg{\ifmmode\mu\tx{g}\else$\mu$g\fi\xspace}
\newcommand\mA{\ifmmode\mu\tx{A}\else$\mu$A\fi\xspace}
\newcommand\mV{\ifmmode\mu\tx{V}\else$\mu$V\fi\xspace}
\newcommand\mF{\ifmmode\mu\tx{F}\else$\mu$F\fi\xspace}
\newcommand\mC{\ifmmode\mu\tx{C}\else$\mu$C\fi\xspace}
\newcommand\mO{\ifmmode\mu\Omega\else$\mu\Omega$\fi\xspace}

\def\lr{%
%\langle\text{\ ,\ }\rangle
{\arraycolsep=3pt%
\begin{array}{ccc}%
\langle & \text{,} & \rangle%
\end{array}}%
}

\def\lrb{%
%\langle\text{\ ,\ }\rangle
{\arraycolsep=3pt%
\begin{array}{ccc@{}}%
\{ & \text{,} & \}%
\end{array}}%
}

%%%%%%%%%%%%%%%%
%   Theorems   %
%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}

\def\enu#1{%
\mbox{}\hspace*{0.5cm}%
\begin{minipage}[t]{12cm}%
\begin{enumerate}\itemsep=-3pt%
#1%
\end{enumerate}%
\vspace{4pt}%
\end{minipage}%
}

\endinput
%%
%% End of file `geomdef.tex'.

